How the interplay between power concentration, competition, and propagation affects the resource efficiency of distributed ledgers

Forks in the Bitcoin network result from the natural competition in the blockchain's Proof-of-Work consensus protocol. Their frequency is a critical indicator for the efficiency of a distributed ledger as they can contribute to resource waste and network insecurity. We introduce a model for the estimation of natural fork rates in a network of heterogeneous miners as a function of their number, the distribution of hash rates and the block propagation time over the peer-to-peer infrastructure. Despite relatively simplistic assumptions, such as zero propagation delay within mining pools, the model predicts fork rates which are comparable with the empirical stale blocks rate. In the past decade, we observe a reduction in the number of mining pools approximately by a factor 3, and quantify its consequences for the fork rate, whilst showing the emergence of a truncated power-law distribution in hash rates, justified by a rich-get-richer effect constrained by global energy supply limits. We demonstrate, both empirically and with the aid of our quantitative model, that the ratio between the block propagation time and the mining time is a sufficiently accurate estimator of the fork rate, but also quantify its dependence on the heterogeneity of miner activities. We provide empirical and theoretical evidence that both hash rate concentration and lower block propagation time reduce fork rates in distributed ledgers. Our work introduces a robust mathematical setting for investigating power concentration and competition on a distributed network, for interpreting discrepancies in fork rates -- for example caused by selfish mining practices and asymmetric propagation times -- thus providing an effective tool for designing future and alternative scenarios for existing and new blockchain distributed mining systems.

==> sections/conclusion.tex <==
\section{Conclusions}
% We considered a set of heterogeneous miners, and computed analytically the probability of observing a given time difference between the two smallest mining times by averaging over the distribution of hash rates between miners.  
% On one hand, the model predicts fork rates which are comparable with the empirical stale blocks rate. On the other hand, where the two values differ, i.e. the fraction of forks is lower or higher than the modeled value, it provides an indication that some fundamental conditions of the protocol might be breached, e.g. miners are not acting independently or the propagation times depend on the node that first mined the new block.   
% The model presented provides a fundamental relationship which allows the fast estimation and calibration of natural fork rates in blockchain systems, for arbitrary distributions of hash rates.
% Further work will be devoted to integrate in this framework the modeling of the propagation time, and as a consequence, the modeling of the network propagation process together with the mining process. This will allow not only to flag discrepancies between the real and theoretical fork rates that should emerge based on the distributions of hash rates in a set of independent miners, but also to associate these discrepancies to specific heterogeneous network properties of the miners.

% \begin{itemize}
%     \item we have a mathematical framework that well describes the occurrence of soft forks and can be used to extrapolate
% 	\item the numbers are consistent with miners being well distributed in the network
% 	\item however we should keep in mind that several of these miners are actually pools, so the aggregation is on a different layer
% 	\item it's unlikely that there are more miners than the ones we see (i.e. zero miners) because we are considering enough B>>N
% 	\item limitations include the stationarity assumption over a relatively long time interval (6.5m) and lack of detail about the dynamics of consensus within pools. also, there is no dynamics over multiple blocks which could affect the results
%     \item while the consensus process in Bitcoin seems to be fair, we still observe a tendency towards concentration of mining power over time that is a potential source of concern.
% \end{itemize}

In this paper we developed a mathematical framework that well describes the occurrence of soft forks in the Bitcoin Proof-of-Work consensus protocol. The model takes as input the hash rate distribution, number of active miners and expected network delay in block propagation to calculate the probability that a soft fork occurs. We explore several specifications of hash rate distributions, considering both ex-ante distributions fitted from empirical mining data and a non-parametric Bayesian empirical distribution. 
% which can then be validated by looking at empirical fork rates as reported in the literature. 

Our study is not exempt from limitations. The most important ones are the lack of detail of intra-pool dynamics and the relatively strong assumption that miners start mining at the same time. While these assumptions were necessary to get to our mathematical description, it is possible that at least some of them could be relaxed and we encourage further research on the topic.

Despite the limitations, we find a good agreement between the predicted fork rates, and in particular that they are consistent with the empirical frequency of soft forks when we consider as propagation delay the time it takes for a block to reach 50\% of nodes in the peer-to-peer network. This would suggest that Bitcoin miners are operating in fair competition, but that most of them have better connectivity than the majority of nodes in the network. Note however that, as most of the miners we consider are actually mining pools, the results would also suggest that cooperation between miners might still be occurring within pools, either through co-location to reduce network delay or by other forms of coordination, as the empirical fork rate is consistent with the model assumption of no intra-pool latency and competition.
%
Beyond its empirical validation, the model formally describes the positive influence of block propagation delay and total mining power over fork rate. It also suggests that a stronger concentration of hash rates---reflected by the fat-tailedness of the distribution---reduces the expected fork rate. 

% However, we should also point out. 
Moreover, we confirm a tendency towards hash rate concentration over time (as shown in \autoref{tab:dists}) which is a potential source of concern. Indeed while this would imply lower fork rates and a more efficient consensus mechanism, it introduces security risks that are not modeled in our framework and that could make the network more vulnerable. Further research is needed to fully explore this trade-off, and we envision our results and methodology to provide a robust mathematical setting for future works in this direction.





==> sections/data.tex <==
\section{Materials and Methods}
\label{sec:data}

\subsection{Data collection and pre-processing}


The mining dynamic in the Bitcoin network naturally changes as miners join and abandon the mining activity.
We thus divide our data chronologically, and consider a period of 20,000 blocks ($\sim$4.5 months) to be approximately stationary. The desired statistics on blocks and miners are then computed period-wise (\autoref{tab:dists}). 

\subsubsection{Block propagation delays}

We obtain propagation times from the Decentralized Systems and Network Services Research Group at KASTEL\footnote{\url{https://www.dsn.kastel.kit.edu/bitcoin/data/invstat.gpd}, accessed 2024-10-13.}---a reputable source often used by related academic works (e.g. \cite{Neudecker2019}), which report the empirical block propagation times to reach 50\%, 90\% and 99\% of the Bitcoin network approximately every hour starting from July 2015. 
% We additionally investigate the possibility of propagation time equal to 8.7s, a previous estimation from~\cite{Fadda2022ConsensusNetworks}.

\subsubsection{Forks} The public GitHub repository \texttt{bitcoin-data/stale-blocks} contains up-to-date, crowd-sourced information on stale blocks and their respective block number. We complement this dataset with anecdotal fork data published by Neudecker et al. \cite{Neudecker2019} and orphan block data from Blockchain.com. 
We then compute the fork rate at a given period as the number of block heights at which at least 1 stale or orphan block appeared, divided by the total number of blocks in that period.
The \texttt{bitcoin-data/stale-blocks} is likely to under-report stale blocks due to its crowd-sourced nature: to reconcile it with other data sources, we adjust the computed fork rate to match the value of 0.41\% reported by Gervais et al. \cite{Gervais2016OnBlockchains} at the end of February 2016. This results in a rescaling of the fork rates by a factor of 1.476. 
 % Existing literature also report similar numbers; for example,  estimate a fork rate of 0.41\% in Februray 2016, in line with our source which shows fork rates to fluctuate between 0.2\% and 0.5\% from late 2015 to early 2016 (see \autoref{subtab:hash_empirical}).

\subsubsection{Miners}

In our framework, a miner can be an independent miner or can be a mining pool. In case of the latter, we assume that there is no propagation delay among the members within the same mining pool. To obtain empirical miner information, we fetch coinbase transaction information including \texttt{block\_time}, \texttt{block\_timestamp} and \texttt{output.addresses} of all the blocks in the Bitcoin blockchain from the public dataset \texttt{crypto\_bitcoin} on Google BigQuery. We then identify blocks mined by mining pools by looking up coinbase trasactions' output addresses on the mining pool dictionary data from \hyperlink{https://www.blockchain.com/explorer/charts/pools}{Blockchain.com} and by looking up the block number on the miner data for selected blocks with forks published by Neudecker et al. \cite{Neudecker2019}\footnote{\url{https://www.dsn.kastel.kit.edu/bitcoin/forks/forks.gpd}, accessed 2024-10-15.}. For the remaining unidentified mining addresses, we use a simple heuristic to cluster: if two addresses ever appear in the same coinbase transaction, we consider them to belong to the same miner (which can be a mining pool). The total number of miners $N$ is thus estimated as the number of those mining clusters.
\autoref{fig:pie} illustrate the distribution of blocks mined among miners throughout time.

\subsubsection{Hash rates}
We retrieve the daily average total hash rate, that is, the average number of hashes per second that can be generated by the aggregate network on a specific day, on the Bitcoin network through the glassnode API\footnote{\url{https://api.glassnode.com/v1/metrics/mining/hash_rate_mean?a=BTC&i=24h}, accessed 2024-10-13.}.
We additionally convert the value of \texttt{bits} of each block fetched from \texttt{crypto\_bitcoin} dataset to the level of mining difficulty (see \autoref{lst:bitcoin_difficulty}); the resultant difficulty value describes the expected number of hashes needed to mine one block. 
For each observation period, the normalized total hash rate $\Lambda$ (in blocks/second) is thus computed as the mean ratio between total hash rate (in hashes/second) and difficulty (in hashes/block). For each period, the calculated $\Lambda$ value equals approximately the reciprocal of block time $t_\text{min}$ (see \autoref{subtab:hash_empirical}), which is in accordance with our model description (Eq. \ref{eq:block_time}).

% \begin{align}
% r &= \tfrac{N}{\Lambda}
% \label{eq:expon_rate}
% \\
% \sigma &= \sqrt{\ln{\left[
% 1+(s/\tfrac{\Lambda}{N})^2
% \right]}}
% \\
% \mu &= \ln\tfrac{\Lambda}{N} - \tfrac{\sigma^2}{2}
% \\
% \alpha &= \tfrac{2 s^2}{s^2 - (\tfrac{\Lambda}{N})^2}
% \\
% \ell &= (\alpha -1) \cdot \tfrac{\Lambda}{N}
% \label{eq:lomax_scale}
% \end{align}
%

\subsubsection{Hash rate distribution estimation}

For each period, we count the number of blocks $\{b_i\}$ mined by each distinct miner $i \in \{1,2,...,N\}$, where we recall $\sum_i^N b_i = B = 20,000$. Miners' hash rates $\{\lambda_i\}$ are then estimated as $\{\tfrac{b_i \Lambda}{B}\}$. 
% The mean $m$ and standard deviation $s$ of the hash rates can subsequently be estimated as
% \begin{align}
% m = \tfrac{\Lambda}{N}, \qquad 
% s = \sqrt{\tfrac{\left( \sum_i \left(\tfrac{b_i \Lambda}{B}\right)^2 - N m^2\right)}{N}}
% =
% \sqrt{\tfrac{\left( \sum_i \left(\tfrac{b_i \Lambda}{B}\right)^2 - \frac{\Lambda^2}{N}\right)}{N-1}}. 
% \end{align}%
We can then apply the method of moments to estimate the parameters the null distributions presented in \autoref{sec:null} from the empirical mean $m = \tfrac{\Lambda}{N}$ and standard deviation $s = \sqrt{\mathrm{Var}\tfrac{b_i\Lambda}{B}}$; specifically, the rate parameter $r$ of $\text{Exp}(r)$,
$\mu$ and $\sigma$ of $\text{LN}(\mu, \sigma^2)$, 
% the shape parameter $c$ and scale parameter $\ell$ of $\text{Lomax}(c, \ell)$,
as well as 
$\alpha$ and $\beta$ of truncated power law $\text{TPL}(\alpha, \beta)$ (see \autoref{sec:null}) are estimated as follows:%
\begin{align}
r = \tfrac{1}{m}
\quad
\sigma = \sqrt{\ln{\left[
1+(\tfrac{s}{m})^2
\right]}}
\quad
\mu = \ln m - \tfrac{s^2}{2}
\quad
\alpha = 1 - \left(\tfrac{m}{s}\right)^2
\quad
\beta = \tfrac{m}{s^2}
\label{eq:mom}
\end{align}%
We display the estimated parameters in  \autoref{subtab:hash_dis}.



% \input{exhibits/hash_rate_plots}

% \subsection{Preliminary and exploratory analysis}

% From \autoref{subtab:hash_empirical}, we observe a clear trend of mining power concentration throughout the last decade: the total number of observed miners was around 100 before 2019, with the hash rate share of the largest miner being as low as 13\% in early 2019 at one time (mid 2017), while the miner number decreased to around 35, with the largest one accounting for a 35\% share by early 2024.
% %
% We see from \autoref{fig:pie} the dominance of Chinese mining pools such as F2Pool, BTCC Pool, Antpool and ViaBTC. Since 2022, some of those pools phased out---likely due to the China's Bitcoin Mining Ban in 2021---and US miners such as Foundry USA started to take lead.\footnote{\url{https://www.bbc.co.uk/news/technology-58896545}}

% We illustrate the evolution of the hash rate distribution in \autoref{fig:ccdf_emp}, and observe an increasing level of fat-tailedness with the passage of time, indicating the emergence of \enquote{mega miners} dominating the mining of the Bitcoin network. 
% The displayed distributions all consider i.i.d. hash rates; the null distributions are fitted using the method of moments \eqref{eq:mom}, while the semi-empirical one was computed according to \eqref{eq:plamb_iid}.
% Among the null distributions, log-normal and truncated power law are the closest fit, both able to capture the right tail---with the truncated power law distribution slightly more so---better than exponential. However, the semi-empirical distribution is better at capturing the tail thickness and cut-off.











==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Let us now comment on the results we briefly presented above. In Figure \ref{fig:forkrate_per_delta} we show the dependency of the analytically calculated fork rate from the number of active miners $n$, the propagation delay $\Delta_0$ and the choice of hash rate distribution. The figure shows how a larger and more homogeneous mining market, i.e. large $N$ and thinner-tailed distributions like the log-normal and the exponential, leads to higher fork rates regardless of propagation delay. This behavior is qualitatively identical for any value of $\Delta_0$. However, from a quantitative standpoint it is clear that higher delays generate much higher fork rates, as would be intuitive. This is a clear representation of the typical inefficiency of totally decentralized and equitable systems, where the low concentration of hashing power inevitably leads to redundancy and waste of resources. On the other hand, a strong concentration of mining power - or a smaller number of miners - leads to less competition and as a consequence to a reduced fork rate, i.e. a more efficient albeit unequal and oligopolistic system.

The main advantage of having an analytical model is its flexibility in predicting behaviors outside of the empirically available parameters. For this reason we show in Figure \ref{fig:surface} a generalization of the previous one, including as additional dimensions the block propagation time $\Delta_0$ and the total committed hash rate $\Sigma \lambda$. Each plot shows the surface of fork rates versus $n$ and $\Delta_0$, changing the distribution of hash rates (columns) and the total hash rate (rows). We find that the lower the total hash rate, the higher the tolerance to heavy delays, as can be seen by the smoother gradient in the first row compared with the extremely steep one in the last row. It is also confirmed that the Lomax distribution leads to generally lower fork rates regardless of the combination of parameters, whereas the exponential and log-normal are much more similar.

Importantly, in all the previous results the parameters of the hash rates distributions are the empirical estimates. Thanks to our modeling approach however we can easily relax this condition and explore the landscape of the expected fork rate as function of the distribution parameters. In Figure \ref{fig:forkrate_per_sigma} we show the expected fork rates under the assumption of log-normally distributed hash rates, varying the number of miners in the market and their heterogeneity in computational power, measured by the log-normal distribution's $\sigma$ parameter. On the resulting heat-map, we plot the isoline that is consistent with the empirical estimate of a fork rate of 0.41\%, while the red star indicates the point corresponding to the empirically estimated parameters of the hash rate distribution. We notice that the fork rate that would be implied by the empirical distribution is either much higher (in the cases where the block delay is high, i.e. Figure \ref{fig:forkrate_per_sigma}c-e) or lower (Figure \ref{fig:forkrate_per_sigma}a-b) than 0.41\%. In particular, if we take the delay used in previous works from the literature of $\Delta_0 = 8.7s$, a fork rate of 0.41\% is unreasonably low compared with the one implied by the hash rate distribution. Conversely, using the propagation time for reaching 50\% of the network $\Delta_0 = 0.815s$, we find that no value of $s>0$ can reproduce the fork rate of $0.41\%$. 

==> sections/introduction.tex <==
\section{Introduction}
The Bitcoin protocol \cite{Nakamoto2008Bitcoin:System}, introduced in 2008, is the first and most famous blockchain-based system operating at scale. It consists of an append-only, public and permission-less ledger, the blockchain, which records transactions of the Bitcoin cryptocurrency between pseudonymous addresses. While the ledger is public and any person with an internet connection and the publicly available node software can read its contents, write access to the ledger is secured by a cryptographic puzzle whose solution involves the local inversion of the SHA-256 hash function \cite{Lilly2004DeviceHashing}. 

This puzzle can only be solved through brute-force calculation, and the winner of this race gains the right to append a new set of valid transactions (a block) to the most recent block and to create a predetermined amount of new Bitcoins that they can take as a reward. Engaging in this process is known as Proof-of-Work (PoW) mining, and its operators are called miners. The puzzle's difficulty is periodically and automatically adjusted by the protocol so that on average a solution is found every 10 minutes, which is the target block time of the Bitcoin ledger. 
%
Given this mechanism, write rights are also permission-less in principle: there is no central authority that has the right to censor or deny write access, and overwriting is also not possible thanks to the protocol's reliance on Merkle trees and chained hashes.

However, due to risk management and the strong economies of scale in technology markets \cite{Arthur1994IncreasingEconomy}, the competition for write access favors the players who have enough economic resources to acquire large numbers of sophisticated, purpose-built machines---known as Application-Specific Integrated Circuits or ASICs---which severely outperform commercial CPUs and GPUs in the solution of the PoW puzzle. This economic mechanism naturally pushes retail miners out of the mining market, as they end up having a negligible probability of successfully mining a block with respect to the most equipped and capitalized entities. Large mining operators also aggregate into even larger mining pools as a way to smooth out their reward payout and share the risk associated with the randomness of the PoW protocol.

This emerging concentration leads to a strongly heterogeneous distribution of hash rates, i.e. the hashes per second (H/s) that miners are able to generate. At the time of writing, 2 mining pools produce over 50\% of new Bitcoin blocks\footnote{Source: \url{https://www.blockchain.com/explorer/charts/pools}, accessed 09 February 2024}, which is a proxy for their share of the total hash rate that is being committed to Bitcoin mining. 
%
This is concerning for several reasons: first, if a single entity could control the absolute majority of mining power, it would be able to run a 51\% attack \cite{Avarikioti2019BitcoinMajority}, i.e. to write false information on the blockchain while always producing the longest chain, which is the standard rule by which nodes determine the \enquote{validated} blockchain; second, concentration distorts the fees market, which Bitcoin users have to pay to incentivize the miners to include their transaction in the limited space of the next block; third, it puts major miners in a censorship position, as they could arbitrarily delay the inclusion of specific transactions on the blockchain.

In this paper, we explore the impact of the heterogeneity of the hash rate distribution on the probability of generating soft forks. These situations arise when two miners solve the PoW puzzle almost simultaneously, and then have to compete to be the first to broadcast their block to the majority of other network nodes. This competition is due to the network latency, which in Bitcoin leads to an average propagation time of about 2 seconds to reach 90\% of the network (see \autoref{sec:data}). 
A soft fork \cite{Decker2013InformationNetwork,eyal2014majority}
can be resolved by the competition of the two versions of the block. The block which eventually is not included in the longest chain becomes an \textit{orphaned} block, and its content will not be considered validated.
Soft forks are an inefficiency of the Bitcoin protocol that leads to wasted computational resources (and thus energy), increasing the cost of network operations and its environmental impact. 


We base our modeling approach on previous work by Fadda et al.\cite{Fadda2022ConsensusNetworks}, who investigate the impact of network structure on the generation of soft forks. Our intent is to relax their assumption that all miners are equal, i.e. have the same hash rate, accounting for a more realistic hash rate distribution, while keeping our solution fully analytical to avoid cumbersome simulations. 
We take literature estimates for the frequency of soft forks in the Bitcoin blockchain \cite{Decker2013InformationNetwork}, and compare it with the results of our modeling approach, which takes as input the number of miners and the parameters of the hash rate distribution. 


==> sections/methodology.tex <==
\section{Results}

\input{exhibits/hash_rate_table}

\input{exhibits/miner_pie}

\subsection{Preliminary and exploratory analysis}

From \autoref{subtab:hash_empirical}, we observe a clear trend of mining power concentration throughout the last decade: the total number of observed miners was around 100 before 2019, with the hash rate share of the largest miner being as low as 13\% in early 2019 at one time (mid 2017), while the miner number decreased to around 35, with the largest one accounting for a 35\% share by early 2024.
%
We see from \autoref{fig:pie} the dominance of Chinese mining pools such as F2Pool, BTCC Pool, Antpool and ViaBTC. Since 2022, some of those pools phased out---likely due to the China's Bitcoin Mining Ban in 2021---and US pools such as Foundry USA started to take lead.\footnote{\url{https://www.bbc.co.uk/news/technology-58896545}}


Soft forks occur when two miners find a valid solution almost simultaneously and then compete to broadcast it first to other network nodes.
The fork is due to the interplay between the mining and the propagation process, and in particular when the block propagation time is longer than the difference in mining time between successful miners. 
The block propagation time is the time it takes to distribute information about a new block to a sufficient amount of nodes within the network, while the mining time difference is the time gap between when the fastest miner (Miner 1) and the second fastest miner (Miner 2) manage to mine the same height block. 
A soft fork then occurs when the block propagation time is longer than the mining time difference because Miner 2 will successfully mine a block of the same height and broadcast it before the mined block information from Miner 1 reaches Miner 2, thus starting a competition in the network between the two blocks for the one that will be maintained in the longest chain. %\autoref{fig:ForkGeneration} shows a schematic representation of the soft fork process. 


To simplify the dynamics, we assume that all miners start mining at $t_1$. As shown in the schematic representation in \autoref{fig:ForkGeneration}, at $t_2$ Miner 1 solves the PoW puzzle for block $x$ and starts broadcasting it to the network. By $t_4$, the message has spread to most of the nodes. However, Miner 2 successfully mines the block at $t_3$, which is later than $t_2$ and earlier than $t_4$. Therefore, based on the definition above, the propagation time is $t_4-t_2$, and the time difference is $t_3-t_2$.

%From $t_2$ to $t_4$, the mined information may not have propagated to Miner 2. Therefore, this miner will continue mining block $x$ from $t2$ instead of verifying the propagated block message and moving forward to the next block. At $t3$ the block $x$ is mined also by Miner 2 and Miner 2 will start to broadcast the message to the network.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/ForkGeneration.pdf}
\caption{Fork generation}
\label{fig:ForkGeneration}
\end{figure}

In this scenario, the miners who received the information from Miner 2 first will take this block as a new starting point for further mining, whereas miners who received the message from Miner 1 first will take the block mined by Miner 1 as the starting point. 
The communication happens over a peer-to-peer network and the propagation of information is based on the network of connections: even though Miner 1 propagates its information earlier than Miner 2, it is possible that some of the nodes receive Miner 2's message first, especially when Miner 2 is a more central node \cite{Fadda2022ConsensusNetworks}. This results in a temporary failure of consensus about the state of the blockchain (i.e. the soft fork), which is generally resolved once a few more blocks have been appended to either prong of the chain by the longest-chain rule.

%Finally, from the perspective of the blockchain, black frame blocks are blocks that have been verified on the longest chain, after a new block appending to it, while the grey frame blocks are blocks that have been mined and are currently within the propagation process, before any new block appending to it. The fork appears in the blockchain at $t_3$, which is the time when miner 2 mined the block. Those two blocks at height $x$ are competing until a new block is mined.

In the following, we will make the fundamental assumption that the probability of generating forks can be quantified by calculating the cumulative distribution function of the time difference between the two fastest miners, taking its value at the propagation time. This assumption is akin to saying that mining power and the structure of the peer-to-peer network are locally stationary, and that miners are homogeneously distributed in the network.

\subsection{Modeling consensus propagation in a heterogeneous network}
\label{sec:model}

We assume that 
% each miner's mining activity is independent of others and that 
the number of successful mining events occurring in a fixed time period is Poisson distributed, as the continuous time limit of a Bernoulli process with low enough success probability. Therefore, in our model, the time to successfully mine a block is exponentially distributed, and the probability of a block being mined at time $t$ (assuming $t_1 = 0$) for miner $i$ is
%
\begin{equation}
p_i(t)=\frac{\lambda_i}{e^{\lambda_i t}},
\label{eq:p_i(t)}
\end{equation}
%
where $\lambda_i$ is the hash rate of miner $i$, which denotes the expected number of blocks per unit of time the miner can independently mine (i.e. without the influence of competition).
The minimum time of mining a block $t_{min}$, which is the mining time of Miner 1, is the first order statistic $t_{(1)}$. The corresponding probability distribution function is:
%
\begin{equation}
p_{(1)}(t \vert \{\lambda_i\})=\sum_{i=1}^N \left( p_i(t) \prod_{j \neq i}^N S_j(t) \right) ,
\label{eq:p(1)_1}
\end{equation}
%
where  $\{\lambda_i\} = \{\lambda_1, \dots, \lambda_N\}$, $N$ is the number of miners; $S_j(t) = \sum_t^\infty p_j(t) = \tfrac{1}{e^{\lambda_j t}}$ is the probability that miner $j$' mining time exceeds $t$. 
If we consider exponential distributions of mining times, it reads
%
\begin{equation}
p_{(1)}(t \vert \{\lambda_i\})= \Lambda e^{-\Lambda \cdot t }
\label{eq:p(1)_2} ,
\end{equation}
%
where $\Lambda$ is the aggregate mining power of the network. 
The expected minimum mining time in this case reads
\begin{equation}
\left\langle t_{\text {min }}\right\rangle =\tfrac{1}{\Lambda}.
\label{eq:block_time}
\end{equation}
%
To obtain the time difference distribution of the two fastest miners, we compute the joint distribution of the first and second-order statistics:
%
\begin{equation}
\begin{split}
p\left(t, t' \vert \{\lambda_i\} \right)&= \sum_{i \neq j} \theta\left(t'-t\right) p_i(t) p_j\left(t'\right) \prod_{k \neq i, j}^N S_k(t')
\nonumber\\
&=
\sum_{i \neq j} \frac{\theta\left(t'-t\right) \lambda_i \lambda_j}{e^{\lambda_i\left(t-t'\right)+\sum_k \lambda_k t'}} 
\end{split} ,
\label{eq:p_t,t'}
\end{equation}
%
where $t'$ is the second shortest mining time and $\theta$ is the Heaviside step function, 
\begin{equation}
\theta (t'-t) = \begin{cases}1, & t'-t \geq 0 \\ 0, & t' -t < 0\end{cases} .
\end{equation}
%
% This function is non-zero only when $t'$ is not less than $t$. 
The distribution of time difference can be derived as
%
\begin{align*}
% \begin{split}
p(\Delta=t'-t \vert \{\lambda_i\}) =\int d t d t' \delta ( \Delta-t'+t ) p (t, t' \vert \{\lambda_i\} )
=\frac{\sum_i^N \frac{\lambda_i \sum_{j \neq i}\lambda_j}{e^{\Delta \sum_{j \neq i} \lambda_j}}}{\sum_i^N\lambda_i} ,
% \end{split}
\label{eq:p_delta}
\end{align*}
%
where $\delta(x)$ is the Dirac delta function, that selects only the values of $t'$ and $t$ such that their difference equals $\Delta$.
More formally, this is the conditional probability of time differences for a given set of hash rates: we can then take an ergodic approach and consider the average over different realizations of hash rates, to obtain the unconditional time difference distribution
%
\begin{align}
p(\Delta) = \int_D p(\Delta \vert \{\lambda_i\}) p(\{\lambda_i\}) ,
\end{align}%
%
where $D \subset \mathbb{R}_+^N$.
The probability of a time gap between the two fastest miners smaller than or equal to $\Delta$ can be computed as the cumulative probability $C(\Delta_0) = C(\Delta \leq \Delta_0)$, which is now simply,
%
\begin{align}
\label{eq:cdelta}
    C(\Delta_0) = \int_0^{\Delta_0} p(\Delta) dt
    = 1- \int_D p(\{\lambda_i\})  
    \left( \tfrac{\sum_i^N \tfrac{ \lambda_i}{e^{\Delta_0 \sum_{j \neq i} \lambda_j}}}{\sum_i^N\lambda_i}\right) .
\end{align}%
%
When $\forall i\neq j, \lambda_i \perp \lambda_j$, we can write out $C(\Delta_0)$ as
\begin{align}
\label{eq:cdelta_id}
C(\Delta_0) = 1-  \int_0^\infty  
    \left[
        \sum_i^N 
    \left(
     \int_0^{\infty}\tfrac{\lambda_i p(\lambda_i)d{\lambda_i}}{e^{x\lambda_i}} 
    \prod_{j \neq i}
    \int_0^{\infty} \tfrac{p(\lambda_j)d{\lambda_j}}{e^{(\Delta+x)\lambda_j}}
    \right)
    \right] dx .
\end{align}
The derivation of Eq. \eqref{eq:cdelta} and \eqref{eq:cdelta_id} can be found in Appendix \ref{sec:fr_deriv}.
%
When we impose the additional assumption of identical distribution, i.e. $\{\lambda_i\}$ are i.i.d., we get
\begin{align}
\label{eq:cdelta_iid}
C(\Delta_0) = 1-  N \int_0^\infty  
    \left[\left(
     \int_0^{\infty}\tfrac{\lambda p(\lambda)d{\lambda}}{e^{x\lambda}}\right) 
    \left(
    \int_0^{\infty} \tfrac{p(\lambda)d{\lambda}}{e^{(\Delta_0+x)\lambda}}
    \right)^{N-1}
    \right] dx .
\end{align}

\subsection{Semi-empirical distribution for $\lambda$}
\label{sec:semi-emp}
The calculation above relies on knowledge of $\lbrace \lambda_i \rbrace$, which however is not a publicly available information. What can be measured from blockchain data is $\lbrace b_i \rbrace$, that is the number of blocks mined by miner $i$ in a given set of blocks of size $B = \sum_i b_i$. Hence, we adopt a Bayesian framework in order to account for the uncertainty on the true value of the hash rates conditioned over a given measurement $\lbrace b_i \rbrace$. The likelihood $p(b \vert \lambda)$ of observing $b$ blocks being mined by a miner with hash rate $\lambda$ follows a Gaussian distribution
%assumption is based on considering the miners as sampling independently over different time steps and averaging a given number of blocks in a given fraction of time, this independent processes converge towards a Gaussian distribution for the fraction of time steps in which a given miner has identified a block: 
$
p(b|\lambda) = \tfrac{e^{-\tfrac{\left(b - \gamma \cdot \lambda\right)^2}{2 \gamma \cdot \lambda}}}{\sqrt{2\pi \gamma \cdot \lambda}}
$,
which is in principle unbounded over $b$ but effectively centered around the value $\gamma \cdot \lambda$, where $\gamma=\tfrac{B}{\Lambda}$. 
% $N$ denotes the number of miners observed to have mined at least 1 block.
Applying Bayes theorem and assuming a flat prior, we can introduce the empirical distribution over $\lambda$ conditioned on a given number of mined blocks:%
\begin{align}
\label{eq:plamb}
p(\lambda|b) = \tfrac{e^{-\tfrac{\left(b - \gamma\cdot \lambda \right)^2}{2 \gamma\cdot \lambda}}}{\sqrt{2\pi \lambda/\gamma}}  .
\end{align}
Assuming $\{\lambda_i\}$ are independent (but not necessarily identically distributed), we plug Eq. \eqref{eq:plamb} in \eqref{eq:cdelta_id} to obtain
\begin{align}
\label{eq:cdelta_id_emp}
C(\Delta_0) = 1-  \int_0^\infty  
    \tfrac{
    \sum_i^{N} 
    \left(
     1+b_i \cdot \sqrt{1+\tfrac{2x}{\gamma}}
         \right) e^{B\left(1-\tfrac{2(\Delta_0+x)}{\gamma}\right)+b_i\left(\sqrt{1+\tfrac{2(\Delta_0+x)}{\gamma}} - \sqrt{1+\tfrac{2x}{\gamma}}\right)}
    }{\gamma  \left(\sqrt{1+\tfrac{2x}{\gamma}}\right)^3  \left(\sqrt{1+\tfrac{2(\Delta_0+x)}{\gamma}}\right)^{N-1}} dx .
\end{align}
In the even more specific case of $\lambda_i$ being i.i.d., we can introduce the semi-empirical marginal distribution for $\lambda$ by averaging $p(\lambda|\{b_i\})$ over $\{b_i\}$, finding
\begin{align}
\label{eq:plamb_iid}
p(\lambda|\{b_i\}) = \tfrac{1}{N}\sum_i^N\tfrac{e^{-\tfrac{\left(b_i - \gamma\cdot \lambda\right)^2}{2 \gamma \cdot \lambda}}}{\sqrt{2\pi \lambda/\gamma}} .
\end{align}
And so, plugging Eq. \eqref{eq:plamb_iid} in \eqref{eq:cdelta_iid}, we arrive at
\begin{align}
\label{eq:cdelta_iid_emp}
C(\Delta_0) = 1-  \int_0^\infty  
    \tfrac{
    \sum_i^N 
    \left(
     1+b_i \cdot \sqrt{1+\tfrac{2x}{\gamma}}
     \right) e^{b_i\left(1 - \sqrt{1+\tfrac{2x}{\gamma}}\right)}
    }{\gamma  \left(\sqrt{1+\tfrac{2x}{\gamma}}\right)^3} 
    \left[ 
        \tfrac{
    \sum_i^N 
    e^{b_i \left(1-\sqrt{1+\tfrac{2(\Delta_0+x)}{\gamma}}\right)}
    }{ N  \sqrt{1+\tfrac{2(\Delta_0+x)}{\gamma}}} 
    \right]^{N-1}dx .
\end{align}


\subsection{Null distributions for i.i.d. $\lambda_i$}\label{sec:null}
As an alternative approach to the Bayesian setting described above, we also consider 3 commonly used null distributions for i.i.d. $\{\lambda_i\}$, assuming they can be distributed according to an exponential, log-normal or truncated power law distribution. 

\subsubsection{Exponential}
We select an exponential distribution for its parsimony, as the distribution can be characterized simply by one rate parameter $r$. For $\lambda_i \sim \text{Exp}(r) \; \forall i$, we plug the density function
\begin{align}
% $
p(\lambda_i) = r e^{-r \lambda_i}
% $
\end{align}
into Eq. \eqref{eq:cdelta_iid} and get
\begin{align}
C(\Delta_0) 
& = 1-  N \int_0^\infty  
    \left[\left(
     \int_0^{\infty}\tfrac{\lambda rd{\lambda}}{e^{x\lambda + r \lambda} }\right) 
    \left(
    \int_0^{\infty} \tfrac{rd{\lambda}}{e^{(\Delta_0+x)\lambda+ r \lambda}}
    \right)^{N-1}
    \right] dx
    \\ & 
    = 
    1-  N r^N \int_0^\infty  \tfrac{dx}{(r+x)^2 
    (\Delta_0+r+x)^{N-1}} .
    \label{eg:c_ex}
\end{align}   

\subsubsection{Log-normal} 
A log-normal distribution is frequently observed in systems characterised by unbounded multiplicative (or proportional) growth \cite{Mitzenmacher2004ADistributions}, and there is a large body of literature supporting the view that blockchain consensus protocols are strongly affected by this accumulation dynamics \cite{Gao2024Heterogeneity-Protocol,Makarov2021BlockchainMarket,Campajola2022ThePlatforms,Campajola2022MicroVelocity:Currencies}.
For $\lambda_i \sim \text{LN}(\mu, \sigma^2) \; \forall i$, we integrate numerically after plugging its density function
\begin{align}
p(\lambda_i) = \frac{e^\frac{-(\ln \lambda_i - \mu)^2}{2 \sigma^2}}{\lambda_i \sigma \sqrt{2 \pi}}
\end{align}%
into Eq. \eqref{eq:cdelta_iid}.

\subsubsection{Truncated power law} A truncated power law distribution also known as power law distribution with exponential cut-off, typically emerges in complex systems where proportional growth effects get capped by some natural scale or limit \cite{Burroughs2001Upper-truncatedSystems}. In the specific context of mining, the cap we would see is given by the fact that the total hashrate sums to $\Lambda$, meaning that each individual miner cannot have a hashrate larger than that in a given sample.
This limitation results in a truncation of the power law at the upper end, which is generally captured by multiplying the power law function with a decreasing exponential.
As above, for $\lambda_i \sim \text{TPL}(\alpha, \beta) \; \forall i$, we can plug the density function 
\begin{align}
% p(\lambda) =  \tfrac{c}{\ell \left(1+\tfrac{\lambda}{\ell}\right)^{c+1}}
% and 
p(\lambda_i) =  \tfrac{\beta^{1-\alpha}}{\Gamma(1-\alpha) \cdot \lambda_i^{\alpha} \cdot e^{\beta \lambda_i}}
\end{align}%
into Eq. \eqref{eq:cdelta_iid} and arrive at
\begin{align}
C(\Delta_0) 
& = 1-  N (1-\alpha) \cdot \beta^{N (1-\alpha)}  \int_0^\infty  
    \frac{dx}{
    (\beta + x)^{2-\alpha} \cdot 
    (\Delta_0+ \beta + x)^{(N-1)(1-\alpha)}
    }.
\label{eg:c_tpl}
\end{align}   
%
For succinctness we omit the derivation steps. Note that the truncated power law distribution can be deemed as a generalization of the exponential distribution. Specifically, when $\beta = r$ and $\alpha = 0$, $\text{TPL}(\alpha, \beta)$ can be reduced to $\text{Exp}(r)$.


% \begin{align}
% \label{eq:cdeltaiid_emp}
% C(\Delta_0) = 1-  \int_0^\infty  
%     \tfrac{
%     \sum_i^N 
%     \left(
%      1+b_i \cdot \sqrt{1+\tfrac{2x}{\gamma}}
%      \cdot e^{B(1-\tfrac{2(\Delta_0+x)}{\gamma})+b_i(\sqrt{1+\tfrac{2(\Delta_0+x)}{\gamma}} - \sqrt{1+\tfrac{2x}{\gamma}})}
%     \right)
%     }{\gamma \cdot \left(\sqrt{1+\tfrac{2x}{\gamma}}\right)^3 \cdot \left(\sqrt{1+\tfrac{2(\Delta_0+x)}{\gamma}}\right)^{n-1}} dx .
% \end{align}

==> sections/related.tex <==
%\section{Related work}
% grapped from yuyao's dissertaion -- to be rewritten

The main focus of our research is the relationship between the distribution of computational power among miners, the block propagation process, and the fork rate in distributed consensus systems. 

Decker et al. \cite{Decker2013InformationNetwork} first investigated the fork generation from a network propagation perspective. Their research first verified that the primary cause of the fork is block propagation delay. The authors quantified the probability of the block mining time and fork generation with the assumption that the computational power is uniformly distributed. Remarkably, according to their simple model, the probability of forks was 1.78\%, while their empirical data suggested a probability of 1.69\%. 
Neudecker et al. \cite{Neudecker2019} monitored empirical data and observed that the probability of a block being incorporated into the main chain has a roughly linear relationship with the time that block has been disseminated prior to the competing block.  Shahsavari et al. \cite{Shahsavari2019PerformanceProtocol} extended the fork probability equation further by introducing new factors, such as block size and network conditions, which determine the propagation time. 
The research assumed the block arrivals as a homogeneous Poisson process and utilized theoretical modeling and simulation methods. They found that smaller block sizes and higher bandwidth have the effect of decreasing the fork rate. The model is proven reliable because the monitored empirical fork rate is 0.09\% and the model result is 0.1\%.

Tessone et al. \cite{Tessone2021StochasticConsensus} proposed a stochastic model and performed numerical simulations to investigate the dynamics of blockchain-based consensus. They found that the concentration of mining power exhibits a significant decrease as network latency levels increase. The concentration level was measured by Gini index. Numerical simulations conducted by Liu et al. \cite{Liu2021} showed that fork rate caused by propagation delay increases with $N$.

As for the theoretical approach which is at the basis of our present contribution, Fadda et al. \cite{Fadda2022ConsensusNetworks} estimated the probability of forks by computing analytically the probability that the time difference of the two fastest miners is lower than the propagation delay needed to reach the whole network. Based on the assumption of homogeneous miners, the estimated fork is 1.45\%, which is comparable to the empirical data of 0.41\%. 

Finally, studies on forks are closely related to the growing literature on strategic mining behavior, like selfish mining \cite{Eyal2014MajorityVulnerable}, stubborn mining \cite{Nayak2016StubbornAttack} or other practices \cite{Liu2018OnN-attackers}. Eyal and Sirer \cite{Eyal2014MajorityVulnerable} originally pointed out that the Bitcoin mining protocol is vulnerable to a potential attack where miners withhold their mined blocks, exploiting network delay and hash rate concentration to gain unfair advantages in mining sequences of blocks, rather than single blocks. While detection of the practice has been scarce, recent research \cite{Li2022TwistedMining} has devised a statistical test that finds anomalous activity by miners that would be compatible with strategic mining.

%This kind of fork is defined as a natural fork by \cite{Shahsavari2019PerformanceProtocol}. \cite{Xiao2020} concluded that natural forks have attracted significant scholarly attention. 
%Past research mainly discussed the relationship between block propagation delay and fork generation probability, \cite{Decker2013InformationNetwork}, \cite{Neudecker2019}, \cite{Liu2021}, and mainly considered reducing the delay as a potential method to reduce the fork rate, such as research by \cite{Jiang2021} and \cite{Gebraselase2022}. 
%Several recent studies investigated the dependence of the fork rate on the computational power \cite{Tessone2021StochasticConsensus} and on the number of miners \cite{Liu2021}, as well as the relationship between the distribution of computational power and the viability of malicious strategies such as Selfish Mining \cite{eyal2014majority,Li2022TwistedMining}.

%Fork rates in Bitcoin have been investigated via theoretical modeling, such as in \cite{Decker2013InformationNetwork} and \cite{Shahsavari2019PerformanceProtocol}, through an empirical analysis, such as in \cite{Neudecker2019}, and with simulation studies, as in \cite{Decker2013InformationNetwork} and \cite{Shahsavari2019PerformanceProtocol}. 

%A major issue with the study of competition and fork rates is that there is no accurate fork data because  stale blocks are not stored within the Bitcoin network. 
%Hence, researchers have employed monitoring nodes to gather real-time fork information to prove the reliability of their models by comparing empirical data with the model results. 

==> sections/simulation.tex <==
%\section{Results}
%\label{sec:analyses}



\input{exhibits/forkrate_per_delta}


\subsection{Monte Carlo simulations}
\label{sec:simulation}

% The coinbase transaction data also contains block timestamps, which we use to compute the empirical average block time, and subsequently, estimate the total hash rate $\Lambda$ simply as its inverse (see \autoref{sec:model}).

To validate our analytical derivations, we conduct simulations within a synthetic blockchain environment.
For each round, we initiate the environment with $N \geq 2$ miners, whose hash powers $\{\lambda_i\}_{i = 1, 2, ..., N}$ are randomly sampled from one of the null distributions. 
To simulate the mining process, we generate for each miner $i$ a mining time $t_i$ following an exponential distribution with rate $\lambda_i$, i.e., $t_i \sim \text{Exp}(\lambda_i)$, mimicking the Poisson arrival pattern of mined blocks (see \autoref{sec:model}). We calculate the time difference $\Delta$ between the two fastest miners for each round. A fork is deemed to have occurred if $\Delta$ is below the pre-specified block propagation time $\Delta_0$; otherwise, the round concludes with no fork.
%
% We repeat a substantial number of rounds to ascertain the fork frequencies. 
For a given set of hyper-parameters ($N$, $m$, $s$, $\Delta_0$, distribution of hash power), we iterate for $n$ rounds---where $n$ is sufficiently large ($n=10^7$ in our experiments)---and count the number of rounds with a fork denoted as $n_\text{fork}$. The simulated fork rate is then calculated as the fraction of simulations where a fork occurred, $\frac{n_\text{fork}}{n}$.

In \autoref{fig:forkrate_per_delta}, we superimpose the analytical results  (thin, opaque curves) on the simulated output (thick, transparent curves) for the null distributions---exponential $\text{Exp}(r)$, log-normal $\text{LN}(\mu,\sigma^2)$ and truncated power law $\text{TPL}(\alpha, \beta)$. The distribution parameters are calculated as Eq.~\eqref{eq:mom} at $m=5\times 10^{-5}$ and $s=1\times10^{-4}$, approximately the same level of the mean and standard deviation of hash rates estimated from our last few sample periods (see \autoref{tab:dists}). We also compute the fork rate using the semi-empirical method under the i.i.d. assumption. Specifically, we assume each miner's hash rate is randomly sampled from the same distribution with the PDF estimated following Eq. \eqref{eq:plamb_iid} using the numbers of blocks mined from the 35 miners and the total hash rate $\Lambda = 0.0017 s^{-1}$. The results are plotted in dashed red curves.

\autoref{fig:forkrate_per_delta} shows that our analytical result correctly predicts the simulation with remarkable accuracy regardless of the underlying distribution, and that, holding hash rate mean $m$ and standard deviation $s$ constant, 
the fork rate increases with the number of participating miners and the block propagation delay, as could be expected. 

%The congruence between the simulated and analytical results (demonstrated by a high level of overlap between the transparent and opaque curves in all scenarios) confirms the accuracy of our analytical formulations. 
%

\input{exhibits/hash_rate_plots}

We illustrate the evolution of the hash rate distribution in \autoref{fig:ccdf_emp}, and observe that as time passes the distribution gets more and more skewed towards the right tail, indicating the emergence of \enquote{mega miners} dominating the mining of the Bitcoin network. 
The displayed distributions all consider i.i.d. hash rates; the null distributions are fitted using the method of moments \eqref{eq:mom}, while the semi-empirical one was computed according to \eqref{eq:plamb_iid}.
Among the null distributions, the log-normal and truncated power law are the closest fit, both able to capture the right tail---with the truncated power law distribution slightly more so---better than exponential. However, the semi-empirical distribution is better at capturing the tail thickness and cut-off.

%The fork rates computed using different distributions appear very close, especially at large $N$. When $N$ is small, we can observe $\text{Exp}(r)$ yield the highest fork rate, followed by $\text{LN}(\mu,\sigma^2)$, and then $\text{TPL}(\alpha,\beta)$ although the gap is rather negligible. 
% Furthermore, the distribution of miners' hash power influences the fork rate. Specifically, for identical distribution means, the hash power following an exponential distribution incurs a higher fork rate compared to that following a Log-normal distribution, with the Lomax distribution exhibiting the lowest fork rate.
%The difference can be explained by the shape of those distributions: the capability of reflecting the high likelihood of a big miner increases in the order of semi-empirical, truncated power-law, log-normal, and exponential distributions (see \autoref{fig:ccdf_emp}). This indicates that the concentration of mining power seems to reduce the fork likelihood.
%

% 
% concerning the fork rate across combinations of different block propagation delays, hash rate distributions, and miner counts. The congruence between these two depicted datasets corroborates the accuracy of our analytical formulations. 

\subsection{Data analysis}

In \autoref{fig:forkrate_time_series}, we compare model estimated fork rates using fitted parameters (\autoref{subtab:hash_dis}) with historical fork rates (\autoref{subtab:hash_empirical}). Specifically, each panel shows a different model-estimated fork rate based on whether the block propagation time is assumed to be the network 50th, 90th or 99th percentile.
Interestingly, we find the estimated fork rate is largely consistent with the empirically estimated fork rate when the block propagation time used is the one that is needed to propagate block information to 50\% of the Bitcoin network. The model appears to significantly overestimate forks only before 2018. This is possibly because big miners around that period were geographically concentrated in one area, e.g. China (see \autoref{fig:pie1}), and the communication between them was faster than between any two average nodes, causing the actual fork rate to be lower than estimated using the longer propagation time. Alternatively, it is also possible that non-miner nodes had much worse connectivity on average because of amateur participation to the network, thus leading to high latency for the majority of nodes but low fork rates as miners were already sophisticated enough to have low latency connections.
Consistent with \autoref{fig:forkrate_per_delta}, among null distributions, the exponential $\text{Exp}(r)$ tends to overestimate most, whereas the truncated power-law $\text{TPL}(\alpha,\beta)$ least, with insignificant difference.

We additionally observe that the model-estimated fork rates $C(\Delta_0)$ change proportionally to block propagation time $\Delta_0$ (reported in green in the plot), at least in the range of values we explored. We explore the reason behind this phenomenon in the ensuing sections.  


\input{exhibits/forkrate_time_series}


\input{exhibits/iid}
\subsection{Fork rate under different assumptions}


\subsubsection{Different distributions}

\input{exhibits/forkrate_per_sigma}

In \autoref{fig:id_vs_iid}, we compare the estimated fork rate under the assumptions of pairwise independence and i.i.d. for miner hash rates, by applying Eq. \eqref{eq:cdelta_id}
and \eqref{eq:cdelta_iid} respectively.
The difference is barely distinguishable when the block propagation time $\Delta_0$ is below 250s. At large $\Delta_0$, we see that the estimated fork rate is slightly higher when assuming $\lambda_i$s are independent but not identically distributed than under the i.i.d. assumption. We also see that at relatively small $\Delta_0$, $C(\Delta_0)$'s sensitivity to $\Delta_0$ is almost constant. 

To check the model's robustness, we repeat the computation setting the total hash rate $\Lambda$ to $0.001s^{-1}$, $0.0017s^{-1}$ and $0.005s^{-1}$ and observe an increase in fork rate with the increment of $\Lambda$ for any given $\Delta_0$. 
This is intuitive as the increase of total hash rate effectively reduces the expected time for a block to be mined, which would have the same effect on fork rate as the increase of block propagation time. The simulated fork rate converging to 100\% with sufficiently large $\Delta_0$ and/or large $\Lambda$ also works as a sanity check for the validity of our analytical solution.

% a propagation delay of up to 1000 seconds. 

\subsubsection{Different levels of heterogeneity}
\label{sec:hetero}



We further examine how hash rates heterogeneity, proxied by standard deviation $s$, would affect fork rates.
% Additionally, we examine the influence of the hash power distribution's shape on the fork rate. To this end, we inspect the effects of varying ($\sigma$) of a log-normally distributed hash power across different numbers of miners and block propagation delays. 
In \autoref{fig:hetero}, we illustrate how fork rates change at different $s$ under log-normal and truncated power law distribution of hash rates, varying the number of miners $N$, for a given total hash rate $\Lambda= 0.0017s^{-1}$ across different block propagation times.
We see that the fork rate diminishes as $s$ increases, that is, when the hash power is more concentrated and heterogeneous. 
The number of miners $N$ has a similar effect: the fork rate decreases as $N$ increases, keeping $s$ constant. 
This effect is more apparent under the truncated power law than under the log-normal distribution.
Note that the above-mentioned effect of $N$ is under the condition of constant total hash rate $\Lambda$, which is different from that for \autoref{fig:forkrate_per_delta} where hash rate mean $m$ is held constant.
The blue curve in \autoref{fig:hetero} represents an isoline for a fork rate of 0.01\%, with the red star marking the scenario of the last sample period with $N=35$ and the $s=1\times 10^{-4}$. 
The analytically derived fork rate is close to the recently observed 0.1\% at $\Delta_0=1$ but is above it when $\Delta_0$ is higher. These results are overall consistent with \autoref{fig:forkrate_per_delta} and \autoref{fig:forkrate_time_series}.

In sum, \autoref{fig:hetero} shows the offsetting effects on fork rate from a decreasing number of miners $N$ and increasing miner hash rate $s$. This explains why in \autoref{fig:forkrate_time_series} it appears that the block propagation time $\Delta_0$ is the only driver on model-estimated fork rates-- it is because historically $N$ and $s$ have been moving in opposite directions (see \autoref{subtab:hash_empirical}) and their respective effects on estimated fork rates have been canceling out.






\subsubsection{Different number of \enquote{zero miners}}
\label{sec:zero}

\input{exhibits/hash_rate_zerominer}

When estimating hash rates from mined block frequencies, we may need to consider the possibility of existent miners that have not been able to mine a block in the period, who we term as \enquote{zero miners}.
In general, assuming a fair sampling, the probability of mining should be simply proportional to the hash rate and the inability of a miner to mine in a long time horizon should reflect a very low hash rate. Nevertheless it is possible, though improbable, that there exists a number of unlucky miners that did not manage to mine a block in a relatively long fraction of time.
In \autoref{fig:zerodist}, we depict the scenarios of different numbers of zero miners being added to the miners observed from our last sample period (\autoref{fig:lastperiod}). For a given number of zero miners, we refit the distributions under the i.i.d. assumption. 
%
The fork rates calculated with the refitted distribution with different numbers of zero miners $N_0$ are depicted in \autoref{fig:surface_emp_iid}-\ref{fig:surface_lomax}.

We additionally check the scenario with miner hash rates following independent, but non-identical distributions applying the semi-empirical approach.
% In order to account for this possibility and test our results against the presence of such miners, we introduce the distribution of zero miners and we investigate two kinds of mixture distributions. 
% 
The distribution of a zero miner's hash rate is essentially
% the marginal distribution of hash rates that is compatible with a zero observed mined block, namely 
the posterior distribution conditioned on zero blocks, which can be written out by plugging $b=0$ into Eq. \eqref{eq:plamb}:
$
p(\lambda|0) = \tfrac{e^{-\tfrac{\gamma \cdot \lambda}{2}}}{\sqrt{2\pi \lambda/\gamma}}
$. The corresponding result is illustrated in \autoref{fig:surface_emp_id}. Overall, the effect of \enquote{zero miners} is almost negligible regardless of the distribution type used or block propagation delay. 



% Once we introduce this distribution, 
% we perform two experiments to quantify the potential effect of zero miners to fork rates. 
% In the first experiment, we build a mixture model where we effectively add a number of $N_0$ miners who have mined zero blocks in the measured sample and then sample $N+N_0$ from the resulting distribution, i.e. 

% $$
% p(\lambda|\{b\},\{0\}) = \frac{1}{N+N_0}\sum_i^N\frac{e^{-\frac{\left(b_i - B\lambda/\Lambda\right)^2}{2B\lambda/\Lambda}}}{\sqrt{2\pi \Lambda\lambda/B}} + \frac{N_0}{N+N_0}\frac{e^{-B\lambda/2\Lambda}}{\sqrt{2\pi \Lambda\lambda/B}}
% $$

% and then sample $\{\lambda_i\}_{i=1}^{N+N_0} \sim p(\lambda|\{b\},\{0\})$. 

% In the second experiment, we sample directly a given number $N_0$ of zero miners directly from the distribution $p(\lambda|0)$, i.e.  $\{\lambda_0\}_{i=1}^{N_0} \sim p(\lambda|0)$, and then a number $N$ miners from the original distribution, i.e. $\{\lambda\}_{i=1}^{N} \sim p(\lambda|\{b\})$, hence eliminating  fluctuations in the fraction of miners from the two distributions.



\input{exhibits/forkrate_propagation}


